Tool Learning in the Wild: Empowering Language Models as Automatic Tool Agents

Augmenting large language models (LLMs) with external tools has emerged as a promising approach to extend their utility, enabling them to solve practical tasks. Previous methods manually parse tool documentation and create in-context demonstrations, transforming tools into structured formats for LLMs to use in their step-by-step reasoning. However, this manual process requires domain expertise and struggles to scale to large toolsets. Additionally, these methods rely heavily on ad-hoc inference techniques or special tokens to integrate free-form LLM generation with tool-calling actions, limiting the LLM's flexibility in handling diverse tool specifications and integrating multiple tools. In this work, we propose AutoTools, a framework that enables LLMs to automate the tool-use workflow. Specifically, the LLM automatically transforms tool documentation into callable functions, verifying syntax and runtime correctness. Then, the LLM integrates these functions into executable programs to solve practical tasks, flexibly grounding tool-use actions into its reasoning processes. Extensive experiments on existing and newly collected, more challenging benchmarks illustrate the superiority of our framework. Inspired by these promising results, we further investigate how to improve the expertise of LLMs, especially open-source LLMs with fewer parameters, within AutoTools. Thus, we propose the AutoTools-learning approach, training the LLMs with three learning tasks on 34k instances of high-quality synthetic data, including documentation understanding, relevance learning, and function programming. Fine-grained results validate the effectiveness of our overall training approach and each individual task. Our methods are an important step towards the use of LLMs for solving real-world tasks with external tools.

==> preamble/metadata.tex <==
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002951.10003227.10003351</concept_id>
       <concept_desc>Information systems~Data mining</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Data mining}

% \ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}


==> table/prompt.tex <==
\begin{table*}[htbp]
\small \centering
\setlength\tabcolsep{4pt}
\begin{tabular}{@{}p{14cm}@{}}

\hline
\rowcolor{Gainsboro}
\multicolumn{1}{l}{\textit{\textbf{Prompt to enable the tool probing}}} 
\\
In this task, you are a programming engineer. Your task is to test the provided tools, which are provided by the OpenAPI platform to access the web information, e.g., movie and music.
Specifically, you need to write Python code to pass the required arguments to call the tools, getting the execution results of the tools.\\
\\
Here are the OpenAPI Specification of the given tool, including their name, functional description, and argument details.\\
\\
\{tool documentation\}\\
\\
To test the tools, please first propose a clear and detailed query to specify the purpose of your test code, e.g., find a movies named The Matrix. Then provide Python code that can be executed directly to finish your query and get the execution results.\\
\\
Note: please always transform the raw execution results into \textasciigrave str\textasciigrave\ (e.g., json.dumps(response.json(),indent=0)) and print them in your code via \textasciigrave print()\textasciigrave. 
\\
\\
Your query: "formulate your query"\\
Your test code: \\
\textasciigrave \textasciigrave \textasciigrave python\\
def test\_code(param...):\\
~~~~~~~...implement details\\
\#call your `test\_code` function\\
...\\
\# transform the raw execution results into \textasciigrave str\textasciigrave print the execution results\\
\textasciigrave \textasciigrave \textasciigrave\\

\hline
\end{tabular}
\caption{The prompt to enable the}
\label{tab:prompt-grounding}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\small \centering
\setlength\tabcolsep{4pt}
\begin{tabular}{@{}p{14cm}@{}}
% \toprule
% \textbf{Prompt to enable the tool probing}
% \\
\hline
\rowcolor{Gainsboro}
\multicolumn{1}{l}{\textit{\textbf{Prompt to enable the tool probing}}} 
\\
In this task, you are a program reviewer. You should read my code and the error message to identify the reason for my bug. Here is my code: \\
\textasciigrave \textasciigrave \textasciigrave python\\
\{code\}\\
\textasciigrave \textasciigrave \textasciigrave\\
Specifically, my code is to call the following tools to solve the question: "\{question\}".  \\
\\

However, my program encounters the bug:\\
=================\\
\{bug\}\\
=================\\
Please help me to analyze my code and attribute the error message to the specific APIs callings. Note that you should select the tool name that triggers the error from the above tool list as your output.\\
\\
Your output: [the tool name]
\\
\\
\hline
\end{tabular}
\caption{The prompt to enable the}
\label{tab:prompt-grounding}
\end{table*}


